Adapter Shield: A Unified Framework with Built-in Authentication for Preventing Unauthorized Zero-Shot Image-to-Image Generation

With the rapid progress in diffusion models, image synthesis has advanced to the stage of zero-shot image-to-image generation, where high-fidelity replication of facial identities or artistic styles can be achieved using just one portrait or artwork, without modifying any model weights. Although these techniques significantly enhance creative possibilities, they also pose substantial risks related to intellectual property violations, including unauthorized identity cloning and stylistic imitation. To counter such threats, this work presents Adapter Shield, the first universal and authentication-integrated solution aimed at defending personal images from misuse in zero-shot generation scenarios. We first investigate how current zero-shot methods employ image encoders to extract embeddings from input images, which are subsequently fed into the UNet of diffusion models through cross-attention layers. Inspired by this mechanism, we construct a reversible encryption system that maps original embeddings into distinct encrypted representations according to different secret keys. The authorized users can restore the authentic embeddings via a decryption module and the correct key, enabling normal usage for authorized generation tasks. For protection purposes, we design a multi-target adversarial perturbation method that actively shifts the original embeddings toward designated encrypted patterns. Consequently, protected images are embedded with a defensive layer that ensures unauthorized users can only produce distorted or encrypted outputs. Extensive evaluations demonstrate that our method surpasses existing state-of-the-art defenses in blocking unauthorized zero-shot image synthesis, while supporting flexible and secure access control for verified users.

==> sec/sec3_preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

\subsection{Background}
\noindent\textbf{Diffusion Models} are currently the most widely used image generative model, with a training process composed of two decoupled phases: the forward and backward processes. Given an input image $x_0$, the forward process progressively adds standard Gaussian noise to $x_0$ at each timestep $t$ through a Markov chain. The output $x_t$ at each timestep is defined as follows:
\begin{equation}
\begin{aligned}
&x_t=\sqrt{\overline{\alpha}_t}x_0+\sqrt{1-\overline{\alpha}_t}\epsilon, \\
\end{aligned}
\label{eq:1}
\end{equation}
where $\alpha_t=1-\beta_t$, $\overline{\alpha}_t=\prod \limits_{s=1}^t\alpha_s$, and $\epsilon\sim\mathcal{N}(0,\mathbf{I})$. After $T$ steps, the clean input $x_0$ is transformed into pure Gaussian noise. In contrast to the forward process, the backward process employs a learnable neural network $\epsilon_{\theta}(x_{t+1},t)$ to estimate the noise added at the current time step from $x_{t+1}$ and thereby reconstruct the variables at the previous time step, $x_{t}$, through denoising. The network weights $\theta$ of $\epsilon_{\theta}$ are optimized by minimizing the following loss function:
\begin{equation}
\begin{aligned}
&\mathcal{L}_{ucond}(\theta,x_0)=\mathbb{E}_{x_0,t,\epsilon\sim\mathcal{N}(0,\mathbf{I})}||\epsilon-\epsilon_\theta(x_{t+1},t)||^2_2, \\
\end{aligned}
\label{eq:2}
\end{equation}
where $\epsilon$ is the reference noise added in the forward process. 

As an extension of diffusion models, stable diffusion models perform the noise addition and denoising processes in the latent space $\mathcal{Z}$ of a pretrained variational autoencoder~\cite{vae} ($\mathbf{VAE}$), thereby reducing computational costs. By incorporating text prompts as conditional inputs, it enables effective text-guided image generation. The objective of stable diffusion models is formulated as follows:
\begin{equation}
\begin{aligned}
&\mathcal{L}_{cond}(\theta,z_0)=\mathbb{E}_{z_0,t,c,\epsilon\sim\mathcal{N}(0,\mathbf{I})}||\epsilon-\epsilon_\theta(z_{t+1},t,c)||^2_2, \\
\end{aligned}
\label{eq:3}
\end{equation}
where $c$ represents the text prompt condition and $z_0$ denotes the latent variables of the input images.

\noindent\textbf{Diffusion Fine-tuning Methods} involve optimizing all or part of the model weights using a small-scale dataset, enable the generation of content that closely resembles the images used during fine-tuning. DreamBooth is a widely adopted fine-tuning method for stable diffusion models. Given a set of images sharing common characteristics, such as the same facial identity, and a text prompt $c$ containing a specific trigger word, Dreambooth enforces a strong association between the fine-tuning images and the trigger word, enabling the model to generate images of that specific identity in response to the trigger word during inference. In addition, to mitigate model overfitting, DreamBooth adds a regularization term during fine-tuning that uses prior prompts $c'$, text inputs without the trigger word, and corresponding images from the original weights. We define $c$ and $c'$ as ``\textit{a photo of sks person}" and ``\textit{a photo of person}", repectively. The objective of DreamBooth is formulated as follows:
\begin{equation}
\begin{aligned}
\mathcal{L}_{db}(\theta,z_0)=&\mathbb{E}_{z_0,t,t'}||\epsilon-\epsilon_\theta(z_{t+1},t,c)||^2_2 \\
&+\lambda||\epsilon'-\epsilon_\theta(z'_{t+1},t',c')||^2_2. \\
\end{aligned}
\label{eq:4}
\end{equation}
where $\epsilon,\epsilon'\sim\mathcal{N}(0,\mathbf{I})$, $t,t'\in[1,T]$, and $\lambda$ balances the weights of regularization term. 

Low-Rank Adaptation (LoRA) preserves the original model weights by freezing them during training, while selectively fine-tuning low-rank matrices injected into the attention layers. This approach significantly reduces computational overhead and alleviates overfitting risks compared to full-parameter fine-tuning.


\noindent\textbf{Zero-shot Image-to-Image Generation} is recently proposed to capture specific image features from a single reference image without altering the pretrained model weights. These methods employ an image encoder to extract embeddings from the reference image and utilize additional cross-attention layers to incorporate them into designated layers of the UNet architecture.

\begin{figure*}[htbp]
\centering
\includegraphics[width=\textwidth]{sec/images/method.pdf}
\caption{The optimization process of the first layer of protective perturbation in DLADiff. This layer can effectively defense fine-tuning based diffusion model customization.}
\label{fig:pipeline-ft}
\end{figure*}

\subsection{Problem Definition\label{problem_definition}}
Let $\mathcal{X}=\{x_1,x_2,...,x_n\}$ denote a set of personal portrait images requiring protection. Our method aims to generate a protective perturbation $\delta_i$ and generate the perturbed version $x'_i=x_i+\delta_i$ for each image in $\mathcal{X}$, such that the perturbed dataset $\mathcal{X}'$ can be safely published. When unauthorized users access $\mathcal{X}'$ and attempt to use these images for diffusion model customization, the resulting outputs exhibit severely degraded quality, effectively preventing identity theft. We define the dataset perturbation as $\delta^*$. The aforementioned objective can be formulated as follows:
\begin{equation}
\begin{aligned}
&\delta^*=\mathop{\arg\min}\limits_{\delta^*}\ \mathcal{A}(\mathbf{DM_c},\mathcal{X}'),\\
&s.t.\ \ ||\delta^*||_\infty\leq\eta, 
\end{aligned}
\label{eq:5}
\end{equation}
where $\mathbf{DM_c}$ represents the customized diffusion models, $\mathcal{A}$ denotes a metric for evaluating generation quality, e.g. Fréchet Inception Distance~\cite{heusel2017gans} (FID) and Identity Score Matching~\cite{deng2019arcface} (ISM), and $\eta$ is the bound of perturbation. In practice, unauthorized users may employ both fine-tuning and zero-shot methods to customize generated results. Therefore, the perturbation $\delta^*$ must provide defense across both fine-tuning and zero-shot methods. This problem is inherently more challenging than the scenario limited to a single type of diffusion model customization. In the case of fine-tuning methods such as DreamBooth, unauthorized users would apply the loss function defined in Eq.~\ref{eq:4} to fine-tune on $\mathcal{X}'$, under which condition $\mathbf{DM_c}$ can be formulated as $\epsilon_{\theta^*}$. $\theta^*$ is the weights after fine-tuning:
\begin{equation}
\begin{aligned}
\theta^*= \mathop{\arg\min}\limits_{\theta}\sum\limits_{x\in\mathcal{X'}}\mathcal{L}_{db}(\theta,x).
\end{aligned}
\label{eq:6}
\end{equation}
For zero-shot methods, an unknown identity encoder is employed to extract identity embeddings from $\mathcal{X}'$, and $\mathbf{DM_c}$ can accordingly be represented as $\mathbf{IE}$. For convenience and compatibility, pretrained face recognition models such as ArcFace are commonly used as identity encoders.


